Audio Dialogues: Dialogues dataset for audio and music understanding

Existing datasets for audio understanding primarily focus on single-turn interactions (i.e. audio captioning, audio question answering) for describing audio in natural language, thus limiting understanding audio via interactive dialogue. To address this gap, we introduce Audio Dialogues: a multi-turn dialogue dataset containing 163.8k samples for general audio sounds and music. In addition to dialogues, Audio Dialogues also has question-answer pairs to understand and compare multiple input audios together. Audio Dialogues leverages a prompting-based approach and caption annotations from existing datasets to generate multi-turn dialogues using a Large Language Model (LLM). We evaluate existing audio-augmented large language models on our proposed dataset to demonstrate the complexity and applicability of Audio Dialogues. Our code for generating the dataset will be made publicly available. Detailed prompts and generated dialogues can be found on the demo website https://audiodialogues.github.io/.

==> 05discussion.tex <==
In this paper, we propose \texttt{Audio Dialogues} dataset that is significant for advancing audio understanding, particularly in the multi-turn dialogues setting for general audio sounds and music. By leveraging a prompting-based approach and utilizing caption annotations from existing datasets, we have been able to generate a substantial volume of high-quality dialogues suitable for training and evaluating audio-based models.

While \texttt{Audio Dialogues} enables models to engage in interactions with the user, leading to better comprehension and more nuanced responses, there are certain limitations. One limitation is the absence of timestamps in the generated questions and answers. In the future, an interesting direction would be to temporally ground an answer about an audio. Another limitation is the need for strong annotations to generate dialogues from LLMs. A potential future direction to scale the generated data will be to generate detailed meta descriptions from an existing audio understanding model and designing human feedback-based data filtration strategies. 


==> prompts.tex <==
\begin{table*}
    \centering
    \begin{tabular}{|p{16cm}|}
        % Drawing a rectangle
        \hline

\textcolor{blue}{sys prompt:}~Based on the sound events, create a dialogue between you (the assistant) and a person (the user) about the events in the audio. Each dialogue should consist of: \\
1. A user examines the audio, and sends a reasonable and creative message to the assistant. 
2. Once the audio is provided, the assistant thoroughly perceives and comprehends them, responding with helpful answers that provide comprehensive reasoning. Do not include timestamps in the answer provided by the assistant.
3. Considering the past dialogue i.e. the question and the answer in the previous timestep, the user chooses another question or further inquiry.
4. The assistant provides a helpful answer providing comprehensive reasoning regarding the audio content.
\\
The audios are 10 seconds long and the sound events are segmented based on where they occur in the audio.
All the questions asked by the user should be diverse and complex.
\\


\textbf{Example 1:}
~Sound Events: Sound of Ambulance (siren) (High-pitched and wailing): [0.0s-1.0s]; Sound of Traffic noise, roadway noise (Droning, loud and intrusive): [0.0s-10.0s]; Sound of Accelerating, revving, vroom (Highpitched, short and intense): [2.0s-10.0s]; Sound of Generic impact sounds (Loud and sharp): [6.7s-6.8s]. 

\textbf{Dialogue:}
\\
User: What does the audio sound like?\\
Assistant: An ambulance siren echoes while traffic noise fades, and an engine revs.
\\
User: Can you describe in more detail about the engine revs?\\
Assistant: The engine revving is highpitched, short and intense. 
\\
User: From the highpitched sound, can you tell me what vehicle it was?\\ 
Assistant: It is hard to tell this from the information provided.
\\
User: Are there any other events in the audio that might be relevant?\\
Assistant: There is a sound of impact which is very loud and sharp.
\\

\textbf{Example 2:}
~
Sound Events: Sound of Outside, rural or natural: [0.000s-10.000s]; Sound of Liquid: [0.474s-0.680s], [4.249s-5.292s]; Sound of Gurgling, bubbling: [0.474s-0.680s], [4.249s-5.292s]; Sound of Splash, splatter: [1.620s-3.116s]; Sound of Laughter: [2.745s-4.029s], [5.299s-10.000s]; Sound of Chuckle, chortle: [2.752s-4.029s]; Sound of Speech: [4.551s-4.935s]; Sound of Male speech, man speaking: [4.557s-4.935s]; Sound of Belly laugh: [5.292s-10.000s]

\textbf{Dialogue:}
\\
User: What are the main events in the audio?\\
Assistant: Liquid sounds, laughter, speech, and a man speaking can be heard in a rural setting.
\\
User: Is is he speaking to other people?\\
Assistant: As there is sound of laughter present from other people, the man might be speaking to others.
\\
User: Can you explain in more detail about the first event?\\
Assistant: The liquid sounds are more of splashing, thrashing and splattering sounds.
\\
User: Are there other people laughing with him?\\
Assistant: Yes, there are other laughter voices along with that of the man.
\\

Based on the above examples, design a four-turn dialogue between the user and assistant for the example given below. 
The question asked by the user should use pronouns such as `he', `she', `it', `they' and `them' while referring to entities that have already occurred in the past questions or answers.
Format each QA pair in a single line as a JSON dictionary (key ``user'' for question, and ``assistant'' for answer, wrapped with \{ and \}). Do not include any other explanation.
\\
\textbf{Example 3:}\\
\hline

    \end{tabular}
    \caption{}
    \label{tab:audioset_prompt}
\end{table*}
% \end{tcolorbox}




\begin{table*}
    \centering
    \begin{tabular}{|p{16cm}|}
        % Drawing a rectangle
        \hline
% \begin{tcolorbox}[colback=gray!5!white,colframe=gray!75!black]

\textcolor{blue}{sys prompt:}~
Based on the music, create a dialogue between you (the assistant) and a person (the user) about the events in the music audio. Each dialogue should consist of: \\
1. A user examines the music, and sends a reasonable and creative message to the assistant. 
2. Once the music audio is provided, the assistant thoroughly perceives and comprehends them, responding with helpful answers that provide comprehensive reasoning. Do not include timestamps in the answer provided by the assistant.
3. Considering the past dialogue i.e. the question and the answer in the previous timestep, the user chooses another question or further inquiry.
4. The assistant provides a helpful answer providing comprehensive reasoning regarding the music content.
The more complex and diverse the question, the better. You can use the list of questions below while asking questions. 
\\
\textbf{List of questions: 
}
Is it a live recording or a studio recording?\\
% Is there a guitar?\\
Is the guitar acoustic or electric?\\
Is it playing chords, a riff or a solo?\\
What music style or genre is it?\\
What key is it in? \\
How about the time signature?\\
What's the tempo? Slow, Medium or Fast?\\
Does it have vocals?    \\
Is it low pitched or high pitched?\\
Is the person speaking fast or slow?\\
What is the language and accent?\\
What emotion is conveyed by the voice?\\
What are the vocal characteristics of that emotion?\\
% Can you describe each person's acoustic environment?\\
How old is the person likely to be given their vocal characteristics?\\

\textbf{Example 1:}
\\
Music description: House music with a thought provoking message in the beginning that eventually builds up and can be used to create the sense of a social revolution.
 
\textbf{Dialogue:}
\\
User: What type of music is this? \\
Assistant: It is house music with synth and drums and a man speaking at the beginning. 
\\
User: What is his tone while speaking?\\
Example 2: He has an intense and energetic tone in his voice. 
\\
User: Does he speak till the end? \\
Assistant: No, he stops speaking halfway and then it is followed by house music. 
\\
User: What is the source of this music?\\
Assistant: This is electronic music. 
\\
\textbf{Example 2: }
\\
Music description: Energetic bluesy song with a harmonica and horn section in musical dialogue.
\\
\textbf{Dialogue:}
\\
User: What instruments are playing in this music?\\
Assistant: This is a jazzy tune with harmonica, trumpet and drums playing. 
\\
User: Which key is the music playing in?\\
Assistant: The key is A Major. 
\\
User: How will you explain the tempo of this piece?\\
Assistant: The music is bouncy and positive with high beats per minute in the beginning and then changes signature halfway through.
\\
User: What is the source of this music?\\
Assistant: This is fusion jazz as it has elements of bass and synthesizer. 
\\
Based on above examples, design a four-turn dialogue between the user and assistant for the example given below. The question asked by the user should use pronouns such as `he', `she', 'it', 'they' and `them' while referring to entities that have already occurred in the past questions or answers.
Format each QA pair in a single line as a JSON dictionary (key ``user" for question, and ``assistant" for answer, wrapped with \{ and \}). Do not include any other explanation.
\\
\textbf{Example 3:}\\

\hline
    \end{tabular}
    \caption{}
    \label{tab:musiccaps_prompt}
\end{table*}
% \end{tcolorbox}



\begin{table*}
    \centering
    \begin{tabular}{|p{16cm}|}
        % Drawing a rectangle
        \hline
\textcolor{blue}{sys prompt:}~
Based on the description of audios, create a dialogue between you (the assistant) and a person (the user) about the events in the audio. \\

\textbf{Example 1:}
\\
Audio 1: Sound of Car (Engine hum and tire noise.)\\
Audio 2: Sound of Car (Engine hum and tire noise.)
\\
User: What's the common type of background sound in these two audios? \\
Assistant: Both of them have sounds of car and engine humming.

\textbf{Example 2:}
\\
Audio 1: Sound of Male singing (Deep, resonant, and powerful tones.): [0.000s-1.246s], [1.595s-1.851s], [5.437s-8.394s]; Sound of Music (Sound produced by vibrating instruments.): [0.000s-10.000s]; Sound of Shout (Loud, high-pitched, intense vocal sound.): [2.375s-2.910s],\\
Audio 2: Sound of Female singing (High-pitched and melodious tones.): [0.000s-1.484s], [3.295s-7.558s], [7.779s-10.000s]; Sound of Singing (Melodic vocal sounds with pitch variation.): [0.000s-1.979s], [4.516s-5.011s], [7.537s-10.000s]; Sound of Crowd (Loud, diverse, and overlapping sounds.): [0.000s-2.013s], [7.558s-10.000s]; Sound of Music (Sound produced by vibrating instruments.): [0.000s-10.000s]; Sound of Human voice (Unique, complex, dynamic sound.): [9.842s-10.000s],
\\
User: What are the differences between the speech in these two audios?\\
Assistant: The first one is male singing, the second one is a female singing.

\textbf{Example 3:}
\\
Audio 1: This is a Christmas music piece with heavy influences from Celtic music. There is a female vocalist singing melodically as the lead. The melodic background is provided by the strings and the piano and at the same time Celtic instruments that resemble a harp and a dulcimer. There is a calming and positive aura to this piece. It could be playing in the background at a Christmas party. It could also be used in Christmas-themed shows or social media content.\\
Audio 2: This music is a spirited instrumental. The tempo is fast with an animated Piano harmony, synthesizer arrangements, synthesised violins, rhythmic digital drums, funky bass lines and electronic sounds. The music is superimposed over sounds of tapping and rhythmic beeping. The music is happy, perky, upbeat, enthusiastic, lively and spirited.\\
Audio 3: This is a lullaby that features a main melody made with a xylophone that has a bright sound. A sustained piano synth creates a dreamy and sleepy ambience sound. A subtle cello plays single chords that bounce from one beat to the next. This is a song a baby could fall asleep to.\\

User: What are the same and different instruments played in these three music audios?\\
Assistant: Piano appear in all these three music. The differences are that the first music has harp, the second music has synthesizer and violins, and the third music has cello. 
\\
Based on the above examples, design a single-turn between the user and assistant for the example given below. 
The question asked by the user should focus on either the similarities or the differences between the audios given for comparison.
Once the description of audios is provided along with the question, the assistant thoroughly perceives and comprehends them, responding with helpful answers that provide comprehensive reasoning. Do not include timestamps in the answer provided by the assistant.
\\
Format each QA pair in a single line as a JSON dictionary (key "user" for question, and "assistant" for answer, wrapped with \{ and \}). Do not include any other explanation.
\\
\textbf{Example 4:}\\

\hline
    \end{tabular}
    \caption{}
    \label{tab:multiple_audios}
\end{table*}
